Data-Aware Device Scheduling for Federated Edge Learning

Federated Edge Learning (FEEL) involves the collaborative training of machine learning models among edge devices, with the orchestration of a server in a wireless edge network. Due to frequent model updates, FEEL needs to be adapted to the limited communication bandwidth, scarce energy of edge devices, and the statistical heterogeneity of edge devices' data distributions. Therefore, a careful scheduling of a subset of devices for training and uploading models is necessary. In contrast to previous work in FEEL where the data aspects are under-explored, we consider data properties at the heart of the proposed scheduling algorithm. To this end, we propose a new scheduling scheme for non-independent and-identically-distributed (non-IID) and unbalanced datasets in FEEL. As the data is the key component of the learning, we propose a new set of considerations for data characteristics in wireless scheduling algorithms in FEEL. In fact, the data collected by the devices depends on the local environment and usage pattern. Thus, the datasets vary in size and distributions among the devices. In the proposed algorithm, we consider both data and resource perspectives. In addition to minimizing the completion time of FEEL as well as the transmission energy of the participating devices, the algorithm prioritizes devices with rich and diverse datasets. We first define a general framework for the data-aware scheduling and the main axes and requirements for diversity evaluation. Then, we discuss diversity aspects and some exploitable techniques and metrics. Next, we formulate the problem and present our FEEL scheduling algorithm. Evaluations in different scenarios show that our proposed FEEL scheduling algorithm can help achieve high accuracy in few rounds with a reduced cost.

==> includes/bio.tex <==
% \begin{IEEEbiography}
% [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/afaf_taik.pg}}]
% {Afaf Taïk}
% (GS, IEEE) received the B.Eng. degree in software engineering from the Ecole Nationale Supérieure d’Informatique et d’Analyse des Systèmes, Rabat, Morocco in 2018, and a DESS in applied sciences from the Université de Sherbrooke, Canada in 2018. She is currently pursuing her Ph.D. degree in the Department of Electrical and Computer and Electrical Engineering, Université de Sherbrooke, Canada. Her research interests include edge computing, machine learning, and the development of statistical and mathematical methods for distributed systems in wireless networks. 
% \end{IEEEbiography}
% \vspace{-13mm}
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/zoubeir_mlika.jpg}}]{Zoubeir Mlika}
% 	(M, IEEE) received the B.Eng. degree from the Higher School of Communication of Tunis, Tunisia, in 2011, and the M.Sc. and Ph.D. degrees from the University of Quebec at Montreal (UQAM), Canada, respectively in 2014 and 2019. He was an intern at UQAM. He was a visiting research intern with the department of Computer Science at University of Moncton, Canada, between Mar. 2018 and Aug. 2018. From Sept. 2019, he joined the Department of Electrical and Computer Engineering in University of Sherbrooke, Canada as Postdoctoral Fellow. His current research interests include vehicular communications, resource allocation, design and analysis of algorithms and computational complexity.
% \end{IEEEbiography}
% \vspace{-15mm}
% \begin{IEEEbiography}
% %[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/soumaya_cherkaoui.jpg}}]
% {Dr. Soumaya Cherkaoui}
% 	(SM, IEEE) is a Full Professor at Department of Electrical and Computer Engineering of Université de Sherbrooke, Canada which she joined as a faculty member in 1999. Her research and teaching interests are in wireless networks. Particularly, she works on next generation networks Edge computing/Network Intelligence, and communication networks. Since 2005, she has been the Director of INTERLAB, a research group which conducts research funded both by government and industry. Before joining U. Sherbrooke, she worked for industry as a project leader on projects targeted at the Aerospace Industry.  Her work resulted in technology transfer to companies and to patented technology.  She has published over 200 research papers in reputed journals and conferences. She has been on the editorial board of several journals including IEEE JSAC, IEEE Network, and IEEE Systems. Her work was awarded with recognitions including a best paper award at IEEE ICC in 2017. She is currently an IEEE ComSoc Distinguished Lecturer. She is a Professional Engineer in Canada and has been designated Chair of the IEEE ComSoc IoT-Ad hoc and Sensor Networks Technical Committee in 2020.
% \end{IEEEbiography}

